Accuracy on the Line: On the Strong Correlation Between Out-of-Distribution and In-Distribution Generalization

For machine learning systems to be reliable, we must understand their performance in unseen, out-of-distribution environments. In this paper, we empirically show that out-of-distribution performance is strongly correlated with in-distribution performance for a wide range of models and distribution shifts. Specifically, we demonstrate strong correlations between in-distribution and out-of-distribution performance on variants of CIFAR-10 & ImageNet, a synthetic pose estimation task derived from YCB objects, satellite imagery classification in FMoW-WILDS, and wildlife classification in iWildCam-WILDS. The strong correlations hold across model architectures, hyperparameters, training set size, and training duration, and are more precise than what is expected from existing domain adaptation theory. To complete the picture, we also investigate cases where the correlation is weaker, for instance some synthetic distribution shifts from CIFAR-10-C and the tissue classification dataset Camelyon17-WILDS. Finally, we provide a candidate theory based on a Gaussian data model that shows how changes in the data covariance arising from distribution shift can affect the observed correlations.

==> baylearn_intro.tex <==
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/figure1}
    \vspace{-.2cm}
    \caption{
      Out-of-distribution accuracies vs. in-distribution accuracies for a wide range of models, datasets, and distribution shifts.
      \textbf{Top left:} A sketch of the current bounds from domain adaptation
      theory. These bounds depend on distributional distances between
      in-distribution and out-of-distribution data, and they are loose in that
      they limit the deviation away from the y = x diagonal but do not prescribe
      a specific trend within these wide bounds.
      \textbf{Remaining panels:} In contrast, we show that for a wide range of
      models and datasets, there is a precise linear trend between
      out-of-distribution accuracy and in-distribution accuracy. Unlike what we
      might expect from theory, the linear trend does not follow the $y = x$
      diagonal. The different panels represent different pairs of
      in-distribution and out-of-distribution datasets. Within each panel, we
      plot the performances of many different models, with different model
      architectures and hyperparameters.
      These datasets capture a variety of distribution shifts from dataset
      reproduction (\cifartentwo~\citep{lu2020harder},
      \imagenettwo~\citep{recht2019imagenet}); a real-world spatiotemporal
      distribution shift on satellite imagery
      (\fmow~\citep{christie2018functional, koh2020wilds}); using a different
      benchmark test dataset (\cinicten~\citep{darlow2018cinic}); synthetic
      perturbations (\cifartenc~\citep{hendrycks2018benchmarking} and
      \ycb~\citep{calli2015benchmarking}); and a real-world geographic shift in
      wildlife monitoring (\iwildcam~\citep{koh2020wilds, beery2020iwildcam}).
      Interestingly, for \iwildcam, models pretrained on \imagenet follow a
      different linear trend than models trained from scratch in-distribution,
      and we plot a separate trend line for \imagenet pretrained models in the
      \iwildcam panel.
        \vspace{-.5cm}
    }
    \label{fig:main_figure}
\end{figure*}

\section{Introduction}
\label{sec:intro}
Machine learning models often need to generalize from training data to new environments.
A kitchen robot should work reliably in different homes, autonomous vehicles should drive reliably in different cities, and analysis software for satellite imagery should still perform well next year.
The standard paradigm to measure generalization is to evaluate a model on a single test set drawn from the same distribution as the training set.
But this paradigm provides only a narrow \emph{in-distribution} performance guarantee: a small test error certifies future performance on new samples from exactly the same distribution as the training set. % and leaves open how well the model will perform on \emph{out-of-distribution} data.
In many scenarios, it is hard or impossible to train a model on precisely the distribution it will be applied to.
Hence a model will inevitably encounter \emph{out-of-distribution} data on which its performance could vary widely compared to in-distribution performance.
Understanding the performance of models beyond the training distribution therefore raises the following fundamental question: how does out-of-distribution performance relate to in-distribution performance? 

%The predominant way to measure generalization is to evaluate a model on a held-out test set. \ar{We perhaps need to say explicitly that the test set is from the same distribution as the training data. Related to PW's comment below}
%However, a test set only provides a narrow \emph{in-distribution} performance guarantee: a small test error guarantees future performance on new samples from the same distribution as the test set. \pw{Here, we're using ID to mean the same distribution as the test set, but in the rest of the paper, we use ID to mean the same distribution as the training set. Is the implicit assumption here that the test set is i.i.d. to the training set? Or are we claiming that any single test set is insufficient evaluation?}
%In many practical applications, trained models are deployed on \emph{out-of-distribution} data that differ from the available test set.
%This raises the fundamental question of how out-of-distribution performance relates to in-distribution performance.
%\ar{I found this starting paragraph slightly dull.. Maybe move the examples to the start of the paragraph and interweave the concrete examples with the abstract definition of ID and OOD. Might also help to make the last sentence an explicit question rather than a statement. }

Classical theory for generalization across different distributions provides a partial answer~\cite{mansour2009domain,bendavid2010theory}.
For a model $f$ trained on a distribution $D$, known guarantees typically relate the in-distribution test accuracy on $D$ to the out-of-distribution test accuracy on a new distribution $D'$ via inequalities of the form
\[
    | \text{acc}_D(f) - \text{acc}_{D'}(f) | \; \leq \;  d(D, D')
\]
where $d$ is a distance between the distributions $D$ and $D'$ such as the total variation distance.
Qualitatively, these bounds suggest that out-of-distribution accuracy may vary widely as a function of in-distribution accuracy unless the distribution distance $d$ is small and the accuracies are therefore close (see Figure 1 (top-left) for an illustration).
%For current models and distribution shifts naturally occurring in practice, existing bounds are loose, which means that a wide range of accuracies are possible (see Figure 1 (top-left) for an illustration).\pw{Is there a citation for ``existing bounds are loose'', since we don't show this? Relatedly, how real are the bounds in Figure 1 (top-left)? Presumably if you use total variation distance then it's completely vacuous?}
More recently, empirical studies have shown that in some settings, models with similar in-distribution performance can indeed have different out-of-distribution performance~\citep{mccoy2019berts,zhou2020curse,damor2020underspecification}.

In contrast to the aforementioned results, recent dataset reconstructions of the popular CIFAR-10, ImageNet, MNIST, and SQuAD benchmarks showed a much more regular pattern \cite{recht2019imagenet,miller2020effect,qmnist,lu2020harder}.
The reconstructions closely followed the original dataset creation processes to assemble new test sets, but small differences were still enough to cause substantial changes in the resulting model accuracies.
%\pw{I wonder if we should spend another sentence explaining dataset reconstructions (like in the previous version)? Not everyone might know immediately what it means, and if it's a reconstruction, it might not also be obvious that it is a distribution shift. Moving the sentence about the substantial gap between ID and OOD accuracies here might also help to head off skeptical readers who would otherwise think that the distribution shifts in these datasets are very minor/non-existent.}
%In contrast to the aforementioned results, \citet{recht2019imagenet,miller2020effect,qmnist,lu2020harder} recently assembled new test sets for the popular CIFAR-10, ImageNet, MNIST, and SQuAD benchmarks by closely following the original dataset creation processes~\cite{krizhevsky2009learning,deng2009imagenet,mnist,rajpurkar2016squad}.
%\pw{Nit: multiple in-line citet's don't read very well because it's not grammatical when you read it out (the cites are all separated by ;) and the reader gets hit by a long set of citations in the opening sentence, which masks the topic sentence. Could consider just removing the original dataset citations and moving the new ones to the end.} \ar{Nit: the assembly of test sets is not in contrast to the results...slightly awkward sentence}
%These dataset reproductions showed a much more regular pattern:
Nevertheless, the new out-of-distribution accuracies are almost perfectly linearly correlated with the original in-distribution accuracies for a range of deep neural networks.
Importantly, this correlation holds \emph{despite the substantial gap between in-distribution and out-of-distribution accuracies} (see Figure 1 (top-middle) for an example).
However, it is currently unclear how widely these linear trends apply since they have been mainly observed for dataset reproductions and common variations of convolutional neural networks.

We conduct a broad empirical investigation to characterize when precise linear
trends such as in Figure 1 (top-middle) may be expected, and when
out-of-distribution performance is less predictable.  Overall, our results show
a striking linear correlation between the in-distribution and
out-of-distribution performance of many contemporary ML models on multiple
distribution shift benchmarks (see Figure 1).  We show that the linear trends
hold for models ranging from state-of-the-art methods such as convolutional
neural networks, visual transformers, and self-supervised models, to classical
methods like logistic regression, nearest neighbors, and kernel machines.  We
also identify three settings in which the linear trends do \emph{not} occur or
are less regular: some of the synthetic distribution shifts in
\cifartenc~\citep{hendrycks2018benchmarking} (e.g., Gaussian noise), the
\camelyon shift of tissue slides from different
hospitals~\citep{bandi2018camelyon,koh2020wilds}, and a version of \iwildcam
wildlife classification problem with a different in-distribution train-test
split \cite{beery2020iwildcam}.  We analyze these cases in detail via additional
experiments to pinpoint possible causes of the linear trends.


==> intro_udl.tex <==
\begin{figure*}[htp!]
    \centering
    \includegraphics[width=\linewidth]{figures/figure1}
    \vspace{-.3cm}
    \caption{
      Out-of-distribution accuracies vs. in-distribution accuracies for a wide range of models, datasets, and distribution shifts.
      \textbf{Top left:} A sketch of the current bounds from domain adaptation theory. These bounds depend on distributional distances between in-distribution and out-of-distribution data, and they are loose in that they limit the deviation away from the y = x diagonal but do not prescribe a specific trend within these wide bounds (see Section \ref{sec:related_work}).
      \textbf{Remaining panels:} In contrast, we show that for a wide range of
      models and datasets, there is a precise linear trend between
      out-of-distribution accuracy and in-distribution accuracy. Unlike what we
      might expect from theory, the linear trend does not follow the $y = x$
      diagonal. The different panels represent different pairs of
      in-distribution and out-of-distribution datasets. Within each panel, we
      plot the performances of many different models, with different model
      architectures and hyperparameters.
      These datasets capture a variety of distribution shifts from dataset
      reproduction (\cifartentwo, \imagenettwo); a real-world spatiotemporal distribution shift
      on satellite imagery (\fmow); using a different benchmark test dataset
      (\cinicten); synthetic perturbations (\cifartenc and \ycb); and a real-world
      geographic shift in wildlife monitoring (\iwildcam). Interestingly, for
      \iwildcam, models pretrained on \imagenet follow a different linear trend
      than models trained from scratch in-distribution. We explore this more in
      Section~\ref{sec:training_data}.
    }
    \label{fig:main_figure}
\end{figure*}

\section{Introduction}
\label{sec:intro}
The goal of machine learning is to create models that generalize from training data to new environments. \pw{Wonder if this is too strong---seems like one could reasonably aim to also create ML models that operate only in a single environment. Maybe soften it a little bit, like ``Machine learning models often need to generalize from training data to new environments: ...'' or something?}
A kitchen robot should work reliably in different homes, autonomous vehicles should drive reliably in different cities, and analysis software for satellite imagery should still perform well next year.
The standard paradigm to measure generalization is to evaluate a model on a single test set drawn from the same distribution as the training set.
But this paradigm provides only a narrow \emph{in-distribution} performance guarantee: a small test error certifies future performance on new samples from exactly the same distribution as the training set. % and leaves open how well the model will perform on \emph{out-of-distribution} data.
In many scenarios, it is hard or impossible to precisely characterize the training distribution and hence a model will inevitably be applied to \emph{out-of-distribution} data on which its performance could vary widely compared to in-distribution performance. \pw{Not sure what it means to characterize the training distribution. Maybe we could be more direct and just say that it's hard or impossible to train on precisely the data that we would want to test on, or something like that?}
Understanding the performance of trained models beyond specific test sets therefore raises the following fundamental question: how does out-of-distribution performance relate to in-distribution performance? \pw{There's a subtle shift here from the previous discussion about being ``out-of-distribution'' versus the concept of ``specific test sets'' here. We're not claiming that the problem is with using specific test sets, right? But rather that the test sets used are i.i.d? So maybe ``understanding the performance of trained models beyond in-distribution test sets'' or more directly something like ``understanding how models perform in these out-of-distribution settings''?}

%The predominant way to measure generalization is to evaluate a model on a held-out test set. \ar{We perhaps need to say explicitly that the test set is from the same distribution as the training data. Related to PW's comment below}
%However, a test set only provides a narrow \emph{in-distribution} performance guarantee: a small test error guarantees future performance on new samples from the same distribution as the test set. \pw{Here, we're using ID to mean the same distribution as the test set, but in the rest of the paper, we use ID to mean the same distribution as the training set. Is the implicit assumption here that the test set is i.i.d. to the training set? Or are we claiming that any single test set is insufficient evaluation?}
%In many practical applications, trained models are deployed on \emph{out-of-distribution} data that differ from the available test set.
%This raises the fundamental question of how out-of-distribution performance relates to in-distribution performance.
%\ar{I found this starting paragraph slightly dull.. Maybe move the examples to the start of the paragraph and interweave the concrete examples with the abstract definition of ID and OOD. Might also help to make the last sentence an explicit question rather than a statement. }

Classical theory for generalization across different distributions provides a partial answer~\cite{mansour2009domain,bendavid2010theory}.
For a model $f$ trained on a distribution $D$, known guarantees typically relate the in-distribution test accuracy on $D$ to the out-of-distribution test accuracy on a new distribution $D'$ via inequalities of the form
\[
    | \text{acc}_D(f) - \text{acc}_{D'}(f) | \; \leq \;  d(D, D')
\]
where $d$ is a distance between the distributions $D$ and $D'$ such as the total variation distance.
Qualitatively, these bounds suggest that out-of-distribution accuracy may vary widely as a function of in-distribution accuracy unless the distribution distance $d$ is small and the accuracies are therefore close (see Figure 1 (top-left) for an illustration).
%For current models and distribution shifts naturally occurring in practice, existing bounds are loose, which means that a wide range of accuracies are possible (see Figure 1 (top-left) for an illustration).\pw{Is there a citation for ``existing bounds are loose'', since we don't show this? Relatedly, how real are the bounds in Figure 1 (top-left)? Presumably if you use total variation distance then it's completely vacuous?}
More recently, empirical studies have shown that in some settings, models with similar in-distribution performance can indeed have different out-of-distribution performance~\citep{mccoy2019berts,zhou2020curse,damor2020underspecification}.

In contrast to the aforementioned results, recent dataset reconstructions of the popular CIFAR-10, ImageNet, MNIST, and SQuAD benchmarks showed a much more regular pattern \cite{recht2019imagenet,miller2020effect,qmnist,lu2020harder}.
\pw{I wonder if we should spend another sentence explaining dataset reconstructions (like in the previous version)? Not everyone might know immediately what it means, and if it's a reconstruction, it might not also be obvious that it is a distribution shift. Moving the sentence about the substantial gap between ID and OOD accuracies here might also help to head off skeptical readers who would otherwise think that the distribution shifts in these datasets are very minor/non-existent.}
%In contrast to the aforementioned results, \citet{recht2019imagenet,miller2020effect,qmnist,lu2020harder} recently assembled new test sets for the popular CIFAR-10, ImageNet, MNIST, and SQuAD benchmarks by closely following the original dataset creation processes~\cite{krizhevsky2009learning,deng2009imagenet,mnist,rajpurkar2016squad}.
%\pw{Nit: multiple in-line citet's don't read very well because it's not grammatical when you read it out (the cites are all separated by ;) and the reader gets hit by a long set of citations in the opening sentence, which masks the topic sentence. Could consider just removing the original dataset citations and moving the new ones to the end.} \ar{Nit: the assembly of test sets is not in contrast to the results...slightly awkward sentence}
%These dataset reproductions showed a much more regular pattern:
Here, in-distribution accuracy is almost perfectly linearly correlated with out-of-distribution accuracy for a range of deep neural networks.
Importantly, this correlation holds \emph{despite a substantial gap between in-distribution and out-of-distribution accuracies} (see Figure 1 (top-middle) for an example).
However, it is currently unclear how widely these linear trends apply since they have been mainly observed for dataset reproductions and common variations of convolutional neural networks.

In this paper, we conduct a broad empirical investigation to characterize when precise linear trends such as in Figure 1 (top-middle) may be expected, and when out-of-distribution performance is less predictable as in Figure 1 (top-left).
Concretely, we make the following contributions:
\shiori{Since we have lots of contributions, my personal preference would be just to write in prose rather than bullet points, although this is minor. Another thought on style is whether we can emphasize the key difference by saying something like "\textbf{Distribution shifts beyond dataset reproductions.} We find..."}
\pw{I'd also vote for writing in prose; it forces smoother transitions.}
%\begin{itemize}[itemsep=-1pt,topsep=-2pt]
\begin{itemize}
  \item We show that clean \pw{precise? or a different word? just to be consistent with the terminology in the prev para} linear trends occur on a wide range of models, datasets, and distribution shifts (see Figure 1).
  We experiment with models ranging from state-of-the-art methods such as convolutional neural networks, visual transformers, and self-supervised models, to classical methods like logistic regression, nearest neighbors, and kernel machines.
  Importantly, we find that classical methods follow the same linear trend as more recent deep learning architectures.
  \pw{Is is that important that the classical methods are the same? I think we might be able to just combine this with the prev sentence, since this is the first (and most prominent) contribution, and then talk about how we consider different distribution shifts here?}
  \pw{Actually, I wonder if it'd make sense to separate models into a different contribution entirely, or to group it with the second contribution below, since changing architecture seems more similar to changing model hyperparameters than to changing datasets/distribution shifts. And the latter is more interesting of a contribution, I think.}
  We find linear trends on a variety of datasets and tasks including\shiori{Should we re-emphasize that these distribution shifts are not just data reproduction shifts? More generally, in these bullet points, I wonder if it's worth explicitly comparing with prior work just to re-emphasize our contributions. Separately, it's a bit unclear if our main point is about having more datasets vs. more distribution shifts -- both are good points, but the latter seems like a clearer difference wrt prior work to me}
  \pw{+1, I'd also vote for emphasizing it; right now I think it comes across a bit as ``we did the same thing as previous work but just on more examples of these kinds of datasets'', which undersells our work.}
  \begin{itemize}
    \item popular image classification benchmarks (\cifarten \cite{krizhevsky2009learning}, \cifartenone \cite{recht2019imagenet}, \cifartentwo \cite{lu2020harder}, \cifartenc \cite{hendrycks2018benchmarking}, \cinicten \cite{darlow2018cinic}, \stlten \cite{coates2011analysis}, \imagenet \cite{deng2009imagenet}, \imagenettwo \cite{recht2019imagenet}),
    \item a pose estimation testbed (based on \ycb \cite{calli2015benchmarking}),
    \item and two distribution shifts derived from concrete applications of image classification: satellite imagery classification and wildlife classification (the \fmow and \iwildcam variants from WILDS~\citep{christie2018functional,beery2020iwildcam,koh2020wilds}).
  \end{itemize}

\item Besides varying model architecture, we demonstrate that varying model or training hyperparameters, training set size, and training duration all result in models that follow the same linear trend.
\pwside{What precisely is shown in figure 1? Just different model architectures? (It's not clear from the caption, e.g., each point could be a different set of hyperparameters?)}

\item We also identify three settings in which the linear trends do \emph{not} occur or are less regular: some of the synthetic distribution shifts in \cifartenc (e.g., Gaussian noise), the \camelyon shift of tissue slides from different hospitals, and an earlier version of the aforementioned \iwildcam wildlife classification problem \cite{beery2020iwildcam}.\shiori{Since people don't know the different versions of iWildCam, should we say it's a different form of IID split?}
We analyze these cases in detail via additional experiments to pinpoint possible causes of the linear trends.

\item We evaluate a range of models pre-trained on other datasets to study the impact of training data on the linear trends. \pw{I wonder if we can give some context here for why pre-training is an interesting question to look at. Like perhaps say that pre-training could improve robustness because the models are exposed to more and more varied data. However, we find that it's mixed; for \cifarten and \fmow, ..., but for \iwildcam, ...; and this is an interesting direction to follow up on, or something like that.}
In some cases, even pre-trained models follow (nearly) the same linear trends as models trained only on the in-distribution training set.
Two examples are ImageNet pre-trained models on \cifarten and \fmow.
In other cases (e.g., \iwildcam), pre-training yields clearly different relationships between in-distribution and out-of-distribution accuracies.

\item Based on our extensive experiments, we summarize specific phenomena that predictive theories for out-of-distribution generalization should capture.
As a starting point for future development, we provide a candidate theory based on a simple Gaussian data model.
Despite its simplicity, we show that this data model correctly identifies the covariance structure of the distribution shift as an important property contributing to the presence or absence of precise linear trends.\pw{Hmm it was a bit surprising to read this sentence because we haven't talked about covariance structure. Also, we don't look at the covariance structure of any of our real datasets, at least in the main text, right? So is this a statement just about the Gaussian data setting or are we claiming that differences in the covariance structure explain why we see  linear trends in some of our datasets but not others?}
\end{itemize}

Understanding the relationship between in-distribution and out-of-distribution performance is essential for developing reliable machine learning.
Our results raise the intriguing possibility that a diverse range of distribution shifts may share common phenomena despite their different creation mechanisms.
Moreover, the linear trends show that models trained without robustness intervention often achieve substantial out-of-distribution performance and hence form an important baseline for robustness interventions.
We hope that our work serves as a step towards organizing the landscape of distribution shifts and will help guide future research on reliable machine learning.
\pw{ What do you think of something like the following that explicitly talks about working on ID vs OOD?
``Overall, our results show a striking linear correlation between the in-distribution and out-of-distribution performance of many contemporary ML models on existing distribution shift benchmarks.
We emphasize that this does \emph{not} imply that improving ID performance is the only way, or even the best way, to improve OOD performance; it is possible that future models or training methods could substantially improve OOD performance without changing ID performance as much.
However, it suggests that strong gains in ID performance can often translate to strong gains in OOD performance as well.
Our results also raise the intriguing possibility that a diverse range of distribution shifts may share common phenomena despite their different creation mechanisms.
We hope that our work serves as a step towards a better understanding of how distribution shifts affect model performance and therefore how we might train models that are can perform robustly OOD.''
}

% Besides the core scientific question, linear trends between in-distribution and out-of-distribution performance can also serve as a guide for future research on reliable machine learning methods.
% Concretely, we see the following potential prescriptive outcomes from this line of research:
% \pw{It was unclear to me if we are claiming these, or if we are merely illustrating the kinds of conclusions one might draw in future work?}
% \begin{itemize}[itemsep=-2pt,topsep=-2pt]
% \item A strong correlation between out-of-distribution and in-distribution performance can simplify model development since we can focus on a single metric.
% \item If a new training approach stands out from the linear trend that all other models follow, this is strong evidence that the approach holds promise for increasing model robustness.
% \pw{This feels a bit contradictory to the first point; if we're only focusing on a single metric, then we wouldn't find this new training approach? And if we care about finding things that are off the line then it seems like we are not focusing on a single metric.}
% \item Since training models on different data is the only intervention that repeatedly affects the linear trends, this suggests that building better training sets is an important avenue for improving model robustness.
% \pw{As above, I'd suggest clarifying how training on different data changes the shift as opposed to being an exception to the linear trend.}
% \end{itemize}
% All of these guidelines rely on a precise understanding of the relationship between in-distribution and out-of-distribution performance, which we establish in this paper.
% \pw{These paras feel like they might belong to a discussion section, which would also help the paper end less abruptly; do we want to add that?} \ar{+1 I think it might help to move a little bit of this to the contribution around predictive theories..that point felt abrupt to me: what's a predictive theory, why do we expect such a theory exists, and why should we find it}
% \ar{High level comment: i think it's important to call the more data parts ``pretraining'' as Yair suggested..otherwise we cannot call the same x-axis as ID performance.}


\paragraph{Paper outline.} Next, we introduce our main experimental framework that forms the backbone of our investigation.
The following sections instantiate this framework for multiple distribution shifts.
Section \ref{sec:linear_trends} shows results on a wide range of distribution shifts where precise linear trends do occur.
Section \ref{sec:fit_failure} then turns to distribution shifts where the linear trends are less regular or do not exist.
Section \ref{sec:training_data} investigates the role of pretraining in more detail since models pre-trained on a different dataset sometimes -- but not always -- deviate from the linear trends.
After our experiments, Section \ref{sec:theory} presents our theoretical model.
%Section TODO concludes with a discussion of our results, possible implications for research on reliable machine learning, and directions for future work.
\pw{If we need space, I think we can cut this entire paragraph and just refer to the sections when we discuss their respective contributions above.}

\section{Experimental setup}
In each of our main experiments, we consider \pw{contrast? compare? consider sounds a bit like we only ever look at two data distributions in the whole paper} two data distributions.
The first is the training distribution $D$, which  we refer to as ``in-distribution'' (ID).
Unless noted otherwise, all models are trained only on samples from $D$ (the main exception is pre-training on a larger dataset).
We compute ID performance via a held-out test set sampled from $D$.
The second distribution is the ``out-of-distribution'' (OOD) distribution $D'$ that we also evaluate the models on.
    For a loss function $\ell$ (e.g., error or accuracy), we denote the loss of model $f$ on distribution $D$ with $\ell_{D}(f) = \mathbb{E}_{x,y\sim D} \left[ \ell(f(x), y) \right]$.

\paragraph{Experimental procedure.} The goal of our paper is to understand the relationship between $\ell_{D}(f)$ and $\ell_{D'}(f)$ for a wide range of models $f$ (convolutional neural networks, kernel machines, etc.) and pairs of distributions $D, D'$ (e.g., CIFAR-10 and the CIFAR-10.2 reproduction).
Hence for each pair $D, D'$, our core experiment follows three steps:
\begin{enumerate}
  \item Train a set of models $\{ f_1, f_2, \ldots \}$ on samples drawn from $D$.
  Apart from the shared training distribution, the models are trained independently with different training set sizes, model architectures, random seeds, optimization algorithms, etc.
\item Evaluate the trained models $f_i$ on two test sets drawn from $D$ and $D'$, respectively.
\item Display the models $f_i$ in a scatter plot with each model's two test accuracies on the two axes to inspect the resulting correlation.
\end{enumerate}
An important aspect of our scatter plots is that we apply a non-linear transformation to each axis.
Since we work with performance measures bounded in $[0, 1]$, we apply an axis scaling that maps $[0, 1]$ to $[-\infty, +\infty]$ via the probit transform. \ludwig{Should we logit everything?}
The probit transform is the inverse of the cumulative density function (CDF) of the standard Gaussian distribution, i.e., $l_\text{transformed} = \Phi^{-1}(l)$.
Transformations like the probit or closely related logit transform are often used in statistics since a quantity bounded to $[0, 1]$ can only show linear trends for a bounded range.
The linear trends we observe in our correlation plots are substantially more precise with the probit (or logit) axis scaling.

\pwside{Can we clarify where the CIs come from, and also how we treat random seeds? In the main text, each point is a different random seed right?}

We assembled a unified testbed that is shared across experiments and includes a multitude of models ranging from classical methods like nearest neighbors, kernel machines, and random forests to random feature models to a variety of high-performance convolutional neural networks.
Overall, our experiments involved more than 3,000 trained models and 100,000 test set evaluations of these models and their training checkpoints.
Due to the size of these experiments, we defer a detailed description of the
testbed with the specific models and datasets used to Appendix \ref{app:testbed}. Unless otherwise noted, all models are trained from random initialization, and we discuss the role of pre-training in Section~\ref{sec:training_data}.


==> pca.tex <==
\section{Beyond Two Distribution: PCA Analysis}
\label{sec:pca}


==> rebuttal_macros.tex <==
% package includes
\usepackage{enumitem}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{mathtools}
\usepackage{xparse}
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{natbib}
\usepackage{mathabx}

%\usepackage[allfiguresdraft]{draftfigure}  % for faster draft compilation


% Personal note macros
\iftoggle{showtodos}{
\newcommand{\john}[1]{{\todo[color=Orange!10]{John: #1}}}
\newcommand{\rohan}[1]{{\todo[color=Red!10]{Rohan: #1}}}
\newcommand{\yair}[1]{{\todo[color=Blue!10]{Yair: #1}}}
\newcommand{\ludwig}[1]{\todo[color=Green!10]{Ludwig: #1}}
\newcommand{\vaishaal}[1]{{\todo[color=White!10]{Vaishaal: #1}}}
% \newcommand{\pw}[1]{{\todo[color=Purple!10]{PW: #1}}}
\newcommand\pw[1]{{\textcolor{Purple}{[PW: #1]}}}
\newcommand{\ar}[1]{{\textcolor{Sienna}{[AR: #1]}}}
\newcommand{\pl}[1]{{\todo[color=Yellow!10]{PL: #1}}}
\newcommand{\shiori}[1]{{\todo[color=Teal!10]{Shiori: #1}}}
\newcommand{\todogeneric}[1]{{\todo[color=Pink!10]{#1}}}
}{
\newcommand{\john}[1]{\ignorespaces}
\newcommand{\rohan}[1]{\ignorespaces}
\newcommand{\yair}[1]{\ignorespaces}
\newcommand{\ludwig}[1]{\ignorespaces}
\newcommand{\vaishaal}[1]{\ignorespaces}
\newcommand{\pw}[1]{\ignorespaces}
\newcommand{\ar}[1]{\ignorespaces}
\newcommand{\pl}[1]{\ignorespaces}
\newcommand{\shiori}[1]{\ignorespaces}
\newcommand{\todogeneric}[1]{\ignorespaces}
}

% Theorems
\theoremstyle{plain}
\newtheorem{conjecture}{Conjecture}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{observation}{Observation}
\theoremstyle{definition}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem*{example*}{Example}


% Math macros
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert} %
\DeclarePairedDelimiter{\brk}{[}{]}
\DeclarePairedDelimiter{\crl}{\{}{\}}
\DeclarePairedDelimiter{\prn}{(}{)}
\DeclarePairedDelimiter{\nrm}{\|}{\|}
\DeclarePairedDelimiter{\norm}{\|}{\|}
\DeclarePairedDelimiter{\tri}{\langle}{\rangle}
\DeclarePairedDelimiter{\dtri}{\llangle}{\rrangle}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}


\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\R}{\mathbb{R}}
\DeclareMathOperator{\sign}{\mathrm{sign}}
\DeclareMathOperator{\tr}{\mathrm{tr}}
\newcommand{\tra}{\widebar{\tr}}
\newcommand{\err}{\mathrm{err}}

% Dataset names
\newcommand{\cifarten}{CIFAR-10\xspace}
\newcommand{\cifartenone}{CIFAR-10.1\xspace}
\newcommand{\cifartentwo}{CIFAR-10.2\xspace}
\newcommand{\cifartenc}{CIFAR-10-C\xspace}
\newcommand{\cifartencorrupted}{CIFAR-10-Corrupted\xspace}
\newcommand{\fmow}{FMoW\xspace}
\newcommand{\iwildcam}{iWildCam\xspace}
\newcommand{\camelyon}{Camelyon17\xspace}
\newcommand{\imagenet}{ImageNet\xspace}
\newcommand{\imagenettwo}{ImageNet-V2\xspace}
\newcommand{\imagenetc}{ImageNet-C\xspace}
\newcommand{\stlten}{STL-10\xspace}
\newcommand{\cinicten}{CINIC-10\xspace}
\newcommand{\ycb}{YCB-Objects\xspace}

